Convergence Rates of Average-Reward Multi-agent Reinforcement Learning via Randomized Linear Programming

In tabular multi-agent reinforcement learning with average-cost criterion, a team of agents sequentially interacts with the environment and observes local incentives. We focus on the case that the global reward is a sum of local rewards, the joint policy factorizes into agents' marginals, and full state observability. To date, few global optimality guarantees exist even for this simple setting, as most results yield convergence to stationarity for parameterized policies in large/possibly continuous spaces. To solidify the foundations of MARL, we build upon linear programming (LP) reformulations, for which stochastic primal-dual methods yields a model-free approach to achieve \emph{optimal sample complexity} in the centralized case. We develop multi-agent extensions, whereby agents solve their local saddle point problems and then perform local weighted averaging. We establish that the sample complexity to obtain near-globally optimal solutions matches tight dependencies on the cardinality of the state and action spaces, and exhibits classical scalings with respect to the network in accordance with multi-agent optimization. Experiments corroborate these results in practice.

==> Experiments_new.tex <==
\section{Experiments}

In this section, we experimentally evaluate our algorithm's performance in terms of steady-state average reward against Multi-agent centralized primal-dual and independent primal-dual RL training algorithms. In particular, we consider a setting where the need for aggregating the policy learnt by independent agents via consensus or centralized training is emphasized. We have used $ n \times n$ grid based MDPs consisting of $m$ agents where the action set of each agent is given by $\mathcal{A}_{agent} : \{ \mathsf{movement-up}, \mathsf{movement-down}, \mathsf{movement-left}, \\
\mathsf{movement-right}  \}$, thus joint Action space is given by $\mathcal{A} = \mathcal{A}_{agent} \times \mathcal{A}_{agent}$,   and the state set consists of all the blocks $\mathcal{S} = \{ 1, 2, ..., n^2 \} $. In our Mazeworld environment as depicted in \ref{fig:regret_rs_6} specifically for $n=3$ and $m = 2$, the agents receive rewards 8 and 5 respectively when they simulaneously reach the top leftmost corner of the grid. Whereas, they are rewarded (5,10) upon jointly reaching the bottom rightmost corner. We use the same definition of the RL environment for $n=2$. In RMAPD and Independent PD algorithms, once local joint state-action occupancy measures $\mu_1$ and $\mu_2$ have been learnt by agent 1 and agent 2 respectively on $\mathcal{S} \times \mathcal{A}$, we obtain the local policies of agents $i \in \{1,2\}$ for all $s \in \mathcal{S}$ and $a_i \in \mathcal{A}_{agent}$ given by: $   \pi_i(a_i|s) = \sum_{a \in \mathcal{A}} \frac{\mu_{i}({s,(a_i,a_{-i})}}{\sum_{a}\mu_{i}({s,a})}$. Henceforth, we find the joint state-action policy assuming independence among the agents as: $\pi(a|s) = \pi_1(a_1|s) \times \pi_1(a_2|s)$. In our mazeworld environment, we note that for each current state $s \in \mathcal{S}$, for every action $a \in \mathcal{A}$, it is straightforward to determine the next state $s' \in \mathcal{S}$. So, directly using $\pi(a|s)$, we obtain transition matrix $\mathbf{P}(.,.)$, where $\mathbf{P}(s,s')$ is the probability with which joint transition happens from state $s$ to next state $s'$. Now, to obtain the steady-state occupancy probabilities $\mathbf{\mu}_{\infty}$ we solve the following system of equations:
\begin{align}
	& \mathbf{\mu}_{\infty}\mathbf{P} = \mathbf{\mu}_{\infty} \\
	& \mathbf{\mu}_{\infty}^T \mathbf{1} = 1
\end{align}

We compute $\mathbf{\mu}_{\infty}$ and leverage it to find stead-state average reward at each time step. We run 20 independent iterations of RMAPD, Independent PD and Centralized PD for $10^7$ timesteps and plot the reward for $(n = 2, m = 2)$ and $(n = 3, m = 2)$ respectively. We observe that convergence is reach sooner in RMAPD algorithm compared to centralized training; thereby corroborating the larger sample requirement in centralized training as opposed to its decentralized counterpart. Further, the importance of the consensus mechanism of the proposed algorithm is highlighted by the much lower average reward achieved by the Independent PD algorithm.


\begin{figure*}[t!]
	\centering
	\subfigure[Mazeworld environment]{
		\includegraphics[scale = 0.32]{maze2_asymm_rewards.png}
		\label{fig:regret_rs_6}
	}
	\hspace{.1in}
	\subfigure[Mazeworld $n = 2$, $m = 2$]{
		\includegraphics[scale = 0.21]{mazesize=2_numagents=2.png}
		\label{fig:regret_rs_12}
	}
	\hspace{.1in}
	\subfigure[Mazeworld $n = 3$, $m = 2$]{
		\includegraphics[scale = 0.21]{mazesize=3_numagents=2.png}
		\label{fig:regret_gw}
	}    
	\caption{Todo}
	\label{fig:per_agent_regret}
	\vspace{-.1in}
\end{figure*}

